Fair Leader Election for Rational Agents in Asynchronous Rings and Networks

We study a game theoretic model where a coalition of processors might collude to bias the outcome of the protocol, where we assume that the processors always prefer any legitimate outcome over a non-legitimate one. We show that the problems of Fair Leader Election and Fair Coin Toss are equivalent, and focus on Fair Leader Election. Our main focus is on a directed asynchronous ring of $n$ processors, where we investigate the protocol proposed by Abraham et al. \cite{abraham2013distributed} and studied in Afek et al. \cite{afek2014distributed}. We show that in general the protocol is resilient only to sub-linear size coalitions. Specifically, we show that $\Omega(\sqrt{n\log n})$ randomly located processors or $\Omega(\sqrt[3]{n})$ adversarially located processors can force any outcome. We complement this by showing that the protocol is resilient to any adversarial coalition of size $O(\sqrt[4]{n})$. We propose a modification to the protocol, and show that it is resilient to every coalition of size $\Theta(\sqrt{n})$, by exhibiting both an attack and a resilience result. For every $k \geq 1$, we define a family of graphs ${\mathcal{G}}_{k}$ that can be simulated by trees where each node in the tree simulates at most $k$ processors. We show that for every graph in ${\mathcal{G}}_{k}$, there is no fair leader election protocol that is resilient to coalitions of size $k$. Our result generalizes a previous result of Abraham et al. \cite{abraham2013distributed} that states that for every graph, there is no fair leader election protocol which is resilient to coalitions of size $\lceil \frac{n}{2} \rceil$.

==> PODC-2018/macros_camera_ready.tex <==

\usepackage[vlined]{algorithm2e}
\usepackage{times}
\usepackage{url}
\usepackage{latexsym}
\usepackage{amsfonts}
\usepackage{bbm}
\usepackage{cleveref}
\usepackage{amsmath}
\usepackage{enumitem}
\usepackage{changepage}
\usepackage{hyperref}
\usepackage{fullpage}
\usepackage{wrapfig}

\usepackage{graphicx}
\usepackage{float}
\usepackage{amsthm}
\usepackage{thm-restate}






\newcommand{\SectionText}{Section }
\newcommand{\sectionsText}{sections }
\newcommand{\sectionText}{section }
\newcommand{\subsomething}{\subsection}
\newcommand{\SubSomethingText}{Subsection }

% Implement a Mux because we have a different version for the ArXiv content and
% for the paper.
\newcommand{\Variant}[2]{#1}


\graphicspath{ {figures/} }



==> PODC-2018/old-equivalent-problems.tex <==

In this \sectionText we show that the most intuitive problem, of Fair Coin-Toss, can be reduced to Fair Leader Election and to Fair Bit-Consensus. While the opposite
directions seem intuitively true, resilience of such reductions is nontrivial
and we do not know whether it holds.


Recall that a \textit{Fair Leader Election} protocol elects a leader
uniformly, i.e., selects an $outcome\in [n]$ uniformly. A
\textit{Fair Coin-Toss} protocol, selects an $outcome\in \{0, 1\}$
uniformly. Like in Fair Leader Election, a Fair Coin-Toss
protocol is \kunbiased if for every
adversarial deviation of size $k$ for any bit value $ b\in\{0,1\}$
we have $ Pr(outcome=b) < \frac{1}{2} + \epsilon$.

In a fair bit-consensus protocol, each processor receives a bit as an input.
If all processors receive the same input bit $b \in \{0, 1\}$, then the 
outcome is $b$. Otherwise, the outcome is selected uniformly from $\{0, 1\}$.
Intuitively, a fair bit-consensus protocol is \kunbiased if a coalition of size $k$ cannot bias the outcome, given that it cannot do it simply by lying about its
$k$ input bits.
Formally, a fair bit-consensus protocol is \kunbiased if for every coalition of
size $k$, for every inputs vector for the honest processors $v \in \{0,1\}^{n-k}$, such that $v \ne 000..$, we have $Pr(outcome=0) \leq \frac{1}{2} + \epsilon$. Similarly, for every inputs vector $v \ne 111..$, we have $Pr(outcome=1) \leq \frac{1}{2} + \epsilon$.

In this \sectionText we assume for simplicity that the number of processors is a power of $2$, $\log_2(n)$ is integer.
\begin{itemize}
	\item \textbf{Leader Election to Coin-Toss}:
	Given an \kunbiased FLE protocol, we construct a
	$\frac{1}{2}n\epsilon$-$k$-unbiased fair coin toss protocol.\\
	Run leader election to get a leader index $i\in [n]$, then output $i \pmod 2$.
	
	So,
	\[Pr(outcome_{coin}=0)\leq \sum_{i=1;i\pmod 2=0}^{n}(\frac{1}{n}+\epsilon) = \frac{1}{2}+\frac{1}{2}n\epsilon\]
	\item \textbf{Bit-Consensus to Coin-Toss}:
	Second, given an \kunbiased fair bit consensus protocol, we construct an
	$(\epsilon+2^{k-n})$-$k$-unbiased fair coin-toss protocol.\\
	Each processor selects randomly an input bit for itself, then runs an \kunbiased fair bit-consensus protocol using that input.
	
	Given an adversarial coalition, denote the inputs selected by honest processors as $v$. $Pr(v=000..)=2^{k-n}$, therefore for every adversarial deviation
	\[Pr(outcome_{coin}=0) = Pr(outcome_{bit-consensus} = 0) = \]
	\[Pr(outcome_{bit-consensus}=0 ~|~ v\ne000..)Pr(v\ne000..) + 
	Pr(outcome_{bit-consensus}=0 ~|~ v=000..)Pr(v=000..) \]
	\[ \leq \frac{1}{2} + 
	\epsilon + 2^{k-n}\]
\end{itemize}
%



==> PODC-2018/related-work.tex <==

%\subsection{Related Work}

\bigskip \noindent{\bf Related Work:}
%\label{section:RelatedWork}
% Leader election on a ring
Most of our work focuses the fundamental problem of leader election
on a ring. Standard algorithms, which are not fault tolerant were
studied in \cite{chang1979improved,dolev1982n,peterson1982n}. These
classical works, elect the processor with the maximal (or minimal)
id as the leader.

% Fault-tolerance in DC
Fault tolerance in distributed systems under classic assumptions of
Byzantine faults and fail-stop faults has been studied extensively.
For examples refer to the following surveys
\cite{correia2011byzantine,sari2015fault}.
%
Fault models that combine both Byzantine, and rational processors,
where studied in
\cite{aiyer2005bar,moscibroda2006selfish,abraham2006distributed,abraham2008lower}.

% Game-theory in DC
There is a variety of game-theoretic approaches to distributed
computing. A discussion about the basic definitions and a brief
survey can be found in \cite{abraham2011distributed}. A well studied
problem in the intersection of game-theoretic and distributed
computing is secret sharing and multi-party computation
\cite{halpern2004rational,abraham2006distributed,kol2008games,dani2011scalable,fuchsbauer2010efficient,gordon2006rational,lysyanskaya2006rationality}.
Recall that our main procedure is a sub-protocol that performs
secret sharing.

% Other models for leader election & game-theory
Fair leader election, fair coin toss and fair consensus (which is
similar to fair coin toss) were explored in various models. For
example, Afek et al. \cite{afek2017cheating} study a variety of
fairness problems in synchronous networks, Clement et al.
\cite{clementi2017rational} study fair consensus in the Gossip
model, and finally, maybe the most studied problem is coin-toss in
the synchronous full-information model
\cite{ben1990collective,saks1989robust,ajtai1993influence,alon1993coin,zuckerman1996randomness,boppana2000perfect,russell2001perfect}.
Our usage of a non-constructive random function in \PhaseAsyncLead
is inspired by the randomized non-constructive approach suggested by
\cite{alon1993coin}.


==> abstract_thesis.tex <==

\begin{abstract}
We study a game theoretic model where a coalition of
processors might collude to bias the outcome of the protocol, where
we assume that the processors always prefer any legitimate outcome
over a non-legitimate one. We show that the problems of Fair Leader
Election and Fair Coin Toss are equivalent, and focus on Fair Leader
Election.

% directed --> unidirectional
Our main focus is on a directed asynchronous ring of $n$ processors,
where we investigate the protocol proposed by Abraham et al.
\cite{abraham2013distributed} and studied in Afek et al.
\cite{afek2014distributed}. We show that in general the protocol is
resilient only to sub-linear size coalitions. Specifically, we show
that $\Omega(\sqrt{n\log n})$ randomly located processors or
$\Omega(\sqrt[3]{n})$ adversarially located processors can force any
outcome. We complement this by showing that the protocol is
resilient to any adversarial coalition of size $O(\sqrt[4]{n})$.
%
We propose a modification to the protocol, and show that it is
resilient to coalitions of size $\Theta(\sqrt{n})$, by exhibiting
both an attack and a resilience result.

For every $k \geq 1$, we define a family of graphs ${\cal{G}}_{k}$
that can be simulated by trees where each node in the tree simulates
at most $k$ processors. We show that for every graph in
${\cal{G}}_{k}$, there is no fair leader election protocol that is
resilient to coalitions of size $k$. Our result generalizes a
previous result of Abraham et al. \cite{abraham2013distributed} that
states that for every graph, there is no fair leader election
protocol which is resilient to coalitions of size $\lceil \frac{n}{2} \rceil$.
\end{abstract}

==> acknowledgements.tex <==

I would like to thank my advisor, Yishay Mansour for his patience to my 
enthusiasm, for his technical insights that saved me decades of redundant work 
and just for being awesome. In addition, I would like to thank my family and 
friends for discussing my ideas with me. Last, I would like to thank Yehuda 
Afek and Moshe Sulamy for introducing the problem to me.


==> macros_thesis.tex <==

\newcommand{\SectionText}{Chapter }
\newcommand{\sectionsText}{chapters }
\newcommand{\sectionText}{chapter }
\newcommand{\subsomething}{\section}
\newcommand{\mySection}{\chapter}
\newcommand{\SubSomethingText}{Section }

